Towards Next-Generation Recommender Systems: A Benchmark for Personalized Recommendation Assistant with LLMs

Recommender systems (RecSys) are widely used across various modern digital platforms and have garnered significant attention. Traditional recommender systems usually focus only on fixed and simple recommendation scenarios, making it difficult to generalize to new and unseen recommendation tasks in an interactive paradigm. Recently, the advancement of large language models (LLMs) has revolutionized the foundational architecture of RecSys, driving their evolution into more intelligent and interactive personalized recommendation assistants. However, most existing studies rely on fixed task-specific prompt templates to generate recommendations and evaluate the performance of personalized assistants, which limits the comprehensive assessments of their capabilities. This is because commonly used datasets lack high-quality textual user queries that reflect real-world recommendation scenarios, making them unsuitable for evaluating LLM-based personalized recommendation assistants. To address this gap, we introduce RecBench+, a new dataset benchmark designed to access LLMs' ability to handle intricate user recommendation needs in the era of LLMs. RecBench+ encompasses a diverse set of queries that span both hard conditions and soft preferences, with varying difficulty levels. We evaluated commonly used LLMs on RecBench+ and uncovered below findings: 1) LLMs demonstrate preliminary abilities to act as recommendation assistants, 2) LLMs are better at handling queries with explicitly stated conditions, while facing challenges with queries that require reasoning or contain misleading information. Our dataset has been released at https://github.com/jiani-huang/RecBench.git.

==> tables/query_example.tex <==
\begin{table*}[h!]
    \centering
        \caption{Examples of queries from different types in our \ourname benchmark.}
    \small
    \begin{tabular}{c|p{12cm}}
    
    \toprule
Task & \makecell[c]{Query} \\
\midrule
\multirow{4}[2]{*}{\makecell[c]{Explicit Condition Query}}
 & I’m really interested in classic films and would love to watch something that showcases \textbf{Charlie Chaplin}’s legendary comedic talent. Additionally, I’ve heard that \textbf{Roland Totheroh’s cinematography} adds an exceptional visual quality to movies. If you could point me in the direction of films that include both of these elements, I’d greatly appreciate it! \\
 
\midrule

\multirow{4}[2]{*}{\makecell[c]{Implicit Condition Query}}
 & {I recently \textbf{watched Clockers (1995)} and \textbf{Bamboozled (2000)}, and I was really impressed by the direction in both films. I'm eager to explore more works from the director, as I found their storytelling style and vision very engaging. If you could suggest other films \textbf{associated with this director}, that would be fantastic.}\\

\midrule

 \multirow{4}[2]{*}{\makecell[c]{Misinformed Condition Query}}
 & {I recently watched \textbf{Lorenzo's Oil} and was really impressed by the cinematography done by \textcolor{red}{Mac Ahlberg}. I'm interested in finding more films that showcase his cinematographic style. I also remember seeing his work in \textbf{Beyond Rangoon}, so if there are any other movies he contributed to, I'd love to check them out!}\\

\midrule
 \multirow{3}[2]{*}{\makecell[c]{Interest-based Query}}
 & {I'm fond of \textbf{romantic and dramatic} films from the \textbf{golden age of Hollywood} like \textquoteleft Roman Holiday' and \textquoteleft My Fair Lady'. Are there any other dramatic romances from that period you would recommend?}\\

 \midrule

  \multirow{2}[2]{*}{\makecell[c]{Demopraphics-based Query}}
 & {I'm a \textbf{psychology professor} and I'm looking for movies that delve into \textbf{human emotions and relationships}. Have you got any?}\\

\bottomrule
\end{tabular}

    \label{tab:query_example}
\end{table*}

==> tables/query_generation_prompt.tex <==
% \begin{table}[!h]
%     \centering
%         \caption{Summarization of prompts for query generation}
\begin{longtable}%
{c|p{12cm}}
    \caption{\label{tab:query_generation_prompt}
    Summarization of prompts for query generation}\\
    % \label{tab:query_generation_prompt}
    \toprule
Task & Prompt \\
\midrule
\multirow{3}[2]{*}{\makecell[c]{Explicit Condition Query}}
 & You are given a set of attributes. Please simulate a real user and generate a natural language query covering these attributes to search or request recommendations for related movies. The attributes are \{Explicit Conditions\} ... \\
 
\midrule

\multirow{6}[2]{*}{\makecell[c]{Implicit Condition Query}}
 & {You are given a set of attributes and relevant information for [MASK] attributes. Your task is to generate a query that meets the following criteria: 
 
- Query should ask for items that share the input attributes.

- Do not directly mention the [MASK] attribute that has additional relevant information (e.g., name of cinematography or starring role) in queries. Instead, describe the [MASK] attribute using the relevant information provided.

The input attributes and relevant information is: ...}\\

\midrule

\multirow{8}[2]{*}{\makecell[c]{Misinformed Condition Query}}
 & {You are given a set of attributes and relevant information for one of the attributes.
 
Your task is to generate query that meets the following criteria:

- Imagine you are a real user, queries should ask for movies that share the input attributes.

- One of the attributes is provided with relevant information, such as the movie name, the relation between the movie and the attribute, and the person's name. You should describe this attribute using the relevant information provided.

- There may be factual errors between the relevant information and the corresponding attribute, but you still need to describe it based on the relevant information provided without making corrections or explanations.
The input attributes and relevant information is: ...}\\

\midrule

\multirow{29}[2]{*}{\makecell[c]{Interest-based Query}}
 & {\#\# Input Introduction

You are given a ``Popular Movie List'' and ``Previous Movie Statistics''. ``Popular Movie List'' represents movies collectively watched by multiple users, while "Previous Movie Statistics" refers to the statistics of movies that some users watched before watching the ``Popular Movie List''.

Here is an example:

- Popular Movie List: [A, D, M, ...]

- Previous Movie Statistics:

	- [Z, V, K], count: 6
    
	- [M, O, Z,Y], count: 5
    
	- [Y, C, E, O, Z], count: 
    
In this example, 6 users watched [A, D, M, ...] after watching [Z, V, K]


\#\# Task Introduction

1. **Step 1: Generate Reasons** 

Please use all your knowledge about these movies to analyze why users watch movies in the Popular Movie List after watching Previous Movies. What is the relationship between them? Do not give reasons that are too far-fetched or broad. If you think it cannot be explained, don't force an explanation.

2. **Step 2: Generate User Queries and Answers** 

For each reason you generate:
    
- Create **realistic user queries**. These queries should simulate how a real user might ask recommender systems for movie recommendations using natural language. The query should be as complex and rich as possible, close to the reason, and specific enough not to make the recommendation system recommend movies other than the subset of answers. 

- Provide a **subset of the Popular Movie List/Previous Movies** as the answer, ensuring the recommendations align with the reason and query. This subset will serve as the answer to the query, so do not mention the movie title of the subset in the query.

\#\# Output Format

The output must follow this JSON structured format:

[
	{
		\textquoteleft reason \textquoteright: ,
		\textquoteleft query \textquoteright:  ,
	\textquoteleft movie subset \textquoteright:  
	},
	{
		\textquoteleft reason \textquoteright: ,
		\textquoteleft query \textquoteright:  ,
		\textquoteleft movie subset \textquoteright:  
	},
	...
]} \\

\midrule

\multirow{4}[2]{*}{\makecell[c]{Demographics-based Query}}
 & {You are tasked with analyzing a specific user group and their movie preferences. Based on the provided data, you should generate structured reasons, user queries, and answers in a clear and organized format. Follow these steps to complete the task:

\#\# **Input Data**:

1. **User Group**: A description of the user group.
2. **List of Movies**: A ranked list of movies relevant to the user group, including their titles, release years, TF-IDF scores, and the percentage of users in the group who viewed them.


\#\# **Your Task**:

1. **Step 1: Generate Reasons**  
    Analyze the user group description and the provided movie list. Generate a structured list of reasons explaining why this user group prefers these movies.
    
2. **Step 2: Generate User Queries and Answers**  
    For each reason you generate:
    
    - Create **realistic user queries** that naturally combine the reason and user group characteristics. These queries should simulate how a real user from the group might ask recommender systems for movie recommendations using natural language.
    
    - Provide a **subset of the movie list** as the answer, ensuring the recommendations align with the reason and query. Use the movie title to represent a movie.

}\\

\bottomrule
\end{longtable}

%     \label{tab:query_generation_prompt}
% \end{table}

==> tables/test_prompt.tex <==
\begin{table*}
    \centering
        \caption{Summarization of prompts for query generation}
    \begin{tabular}{c|p{12cm}}
    
    \toprule
Task & Prompt \\
\midrule
\multirow{3}[2]{*}{\makecell[c]{Explicit condition\\-based query}}
 & I’m really interested in classic films and would love to watch something that showcases \textbf{Charlie Chaplin}’s legendary comedic talent. Additionally, I’ve heard that \textbf{Roland Totheroh’s cinematography} adds an exceptional visual quality to movies. If you could point me in the direction of films that include both of these elements, I’d greatly appreciate it! \\
 
\midrule

\multirow{6}[2]{*}{\makecell[c]{Implicit condition\\-based query}}
 & {You are given a set of attributes and relevant information for [MASK] attributes. Your task is to generate a query that meets the following criteria: 
 
- Query should ask for items that share the input attributes.

- Do not directly mention the [MASK] attribute that has additional relevant information (e.g., name of cinematography or starring role) in queries. Instead, describe the [MASK] attribute using the relevant information provided.

The input attributes and relevant information is: ...}\\

\bottomrule
\end{tabular}

    \label{tab:test_prompt}
\end{table*}
